Safety Aware Changepoint Detection for Piecewise i.i.d. Bandits

In this paper, we consider the setting of piecewise i.i.d. bandits under a safety constraint. In this piecewise i.i.d. setting, there exists a finite number of changepoints where the mean of some or all arms change simultaneously. We introduce the safety constraint studied in \citet{wu2016conservative} to this setting such that at any round the cumulative reward is above a constant factor of the default action reward. We propose two actively adaptive algorithms for this setting that satisfy the safety constraint, detect changepoints, and restart without the knowledge of the number of changepoints or their locations. We provide regret bounds for our algorithms and show that the bounds are comparable to their counterparts from the safe bandit and piecewise i.i.d. bandit literature. We also provide the first matching lower bounds for this setting. Empirically, we show that our safety-aware algorithms perform similarly to the state-of-the-art actively adaptive algorithms that do not satisfy the safety constraint.

==> uai2022.tex <==
In this section we test \glb and \loc against safety oblivious actively adaptive algorithms \glrucb, \ucbcpd as well as passive  algorithm \ducb, and safety aware algorithms \cucb, and \umoss.  
A detailed discussion on the algorithms, hyper-parameter tuning, and time complexity of the algorithms is given in \Cref{app:addl-expt}. 
% Another experiment showing the performance of \sfb vs. \cucb in \emph{no changepoint setting} is shown in \Cref{app:addl-expt}. 
One further experiment showing the performance of \glb, \loc under different values of $\alpha$ is shown in \Cref{app:addl-expt}. All codes are provided in supplementary material. 

\textbf{Global Changepoint:} In this setting all the arms (including baseline) change at every changepoint. The environment consist of $6$ arms (including baseline) and the evolution of means with respect to rounds is shown in \Cref{fig:exptenv} (Left). The three global changepoints are at $t=2000, 4000$ and $6000$. We set risk parameter $\alpha = 0.7$. The performance of all the algorithms is shown in \Cref{fig:expt} (Left). The adaptive algorithms like \ucbcpd, \glrucb perform well as they detecting the changepoints and restart but they do not satisfy the safety constraints. Note that \glb performs similar to \glrucb, \ucbcpd as it also detects the changepoints and restarts as well as satisfy the safety constraint. It outperforms passive algorithm \ducb, and safety aware algorithm \cucb. The safety aware algorithm \cucb is not suited for the safety constraint \eqref{eq:constraint1} under piecewise i.i.d. setting as it always chooses the baseline arm and fail to achieve sub-linear regret. 
% We also implement the \loc algorithm which works for both \gcs and \lcs environment. We see that \loc outperforms passive \ducb but is beaten by \glb which conducts no forced exploration.

\begin{figure}[!ht]
\centering
\begin{tabular}{cc}
\label{fig:global_env}\hspace{-1.2em}\includegraphics[scale = 0.30]{img/global_env.png} &
%%%%%%%%%%
\label{fig:local_env}\hspace{-1.2em}\includegraphics[scale = 0.30]{img/local_env.png}  
\end{tabular}
\caption{(Left) Global changepoint environment with $T=8000$, $K^+ = 6$ and changepoints at $t = 2000, 4000$ and $6000$. (Middle) Local changepoint environment with $T=8000$, $K^+ = 6$ and changepoints at $t = 2000, 4000$ and $6000$. Note that some arms do not change at these changepoints.}
\label{fig:exptenv}
%\vspace{-1.em}
\end{figure}

\begin{figure}[!ht]
\centering
\begin{tabular}{cc}
\label{fig:global}\hspace*{-1.2em}\includegraphics[scale = 0.31]{img/global.png} &
%%%%%%%%%%
\label{fig:local}\hspace*{-1.2em}\includegraphics[scale = 0.31]{img/local.png} 
\end{tabular}
\caption{(Left) \gcs setting with $3$ changepoints and $6$ arms. (Right) \lcs setting with $3$ changepoints and $6$ arms.}
\label{fig:expt}
\vspace{-1.0em}
\end{figure}



\textbf{Local Changepoint:} In this setting at least one arm changes at every changepoint. 
%Note that in this environment the baseline arm does not change at all. 
We show that the environment in \Cref{fig:exptenv} (Right) and the performance of all the algorithms in \Cref{fig:expt} (Right). The three local changepoints are at $t=2000, 4000$ and $6000$. We set a constant baseline $\mu_0 = 0.35$, and risk parameter $\alpha =0.7$. 
Again we see that the safety aware algorithm \cucb fail to achieve sub-linear regret as it always chooses the baseline arm. On the other hand adaptive algorithms like \ucbcpde, \glrucb performs well in detecting the changepoints but they do not satisfy the safety constraints. Note that \glb performs similar to \glrucb, \ucbcpd as it also detects the changepoints and restarts as well as satisfy the safety budget. It outperforms passive algorithm \ducb, and safety aware algorithm \cucb. 


